Feasibility with Language Models for Open-World Compositional Zero-Shot Learning

Humans can easily tell if an attribute (also called state) is realistic, i.e., feasible, for an object, e.g. fire can be hot, but it cannot be wet. In Open-World Compositional Zero-Shot Learning, when all possible state-object combinations are considered as unseen classes, zero-shot predictors tend to perform poorly. Our work focuses on using external auxiliary knowledge to determine the feasibility of state-object combinations. Our Feasibility with Language Model (FLM) is a simple and effective approach that leverages Large Language Models (LLMs) to better comprehend the semantic relationships between states and objects. FLM involves querying an LLM about the feasibility of a given pair and retrieving the output logit for the positive answer. To mitigate potential misguidance of the LLM given that many of the state-object compositions are rare or completely infeasible, we observe that the in-context learning ability of LLMs is essential. We present an extensive study identifying Vicuna and ChatGPT as best performing, and we demonstrate that our FLM consistently improves OW-CZSL performance across all three benchmarks.

==> tables/main_table.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llccc|ccc|ccc}
\toprule
\bf{ViT-L/14} & & \multicolumn{3}{c|}{MIT-States} & \multicolumn{3}{c|}{UT-Zappos} & \multicolumn{3}{c}{C-GQA} \\ \hline
VLM & Method & U & H & AUC & U & H & AUC & U & H & AUC \\
\hline
\multirow{3}{*}{CLIP}
& GloVe
& 14.6 & 13.0 & 3.10
& 19.3 & 10.6 & 1.60 
& \bf 3.92 & 2.46 & \bf 0.20 \\
& ConceptNet
& 12.5 & 12.7 & 2.75 
& 21.3 & 10.3 & 1.69 
& 2.01 & 2.59 & 0.13 \\
& \ours\ (ours)  
% & \bf 16.0 & \bf 14.0 & \bf 3.49
& \bf 16.1 & \bf 13.7 & \bf 3.38
& \bf 23.6 & \bf 11.5 & \bf 1.94
& 2.62 & \bf 2.82 & 0.16  \\
\hline
\multirow{3}{*}{CoOp} 
& GloVe
& 16.7\scriptsize$\pm0.3$ & 16.2\scriptsize$\pm0.4$ & 4.78\scriptsize$\pm0.2$ 
& 36.7\scriptsize$\pm2.4$ & 34.2\scriptsize$\pm3.7$ & 18.1\scriptsize$\pm2.8$ 
& 5.09\scriptsize$\pm0.4$ & 6.16\scriptsize$\pm0.5$ & 1.03\scriptsize$\pm0.1$ \\
& ConceptNet
& 14.5\scriptsize$\pm0.3$ & 15.6\scriptsize$\pm0.3$ & 4.36\scriptsize$\pm0.1$
& 42.1\scriptsize$\pm2.3$ & 36.6\scriptsize$\pm3.2$ & 20.6\scriptsize$\pm2.5$
& 4.14\scriptsize$\pm0.5$ & 5.88\scriptsize$\pm0.7$ & 0.92\scriptsize$\pm0.2$ \\
& \ours\ (ours)  
% & \bf 18.5\scriptsize$\pm0.4$ & \bf 17.5\scriptsize$\pm0.4$ & \bf 5.39\scriptsize$\pm0.1$ 
& \bf 18.7\scriptsize$\pm0.3$ & \bf 17.4\scriptsize$\pm0.5$ & \bf 5.40\scriptsize$\pm0.1$ 
& \bf 49.6\scriptsize$\pm1.7$ & \bf 40.6\scriptsize$\pm3.1$ & \bf 24.4\scriptsize$\pm2.7$
& \bf 5.24 & \bf 6.86 & \bf 1.09 \\
% & \bf 51.82 & \bf 42.25 & \bf 26.68 
% & \bf 5.24 & \bf 7.02 & \bf 1.10 \\
\hline
\multirow{3}{*}{CSP} 
& GloVe
& 14.9\scriptsize$\pm0.3$ & 16.4\scriptsize$\pm0.4$ & 5.12\scriptsize$\pm0.2$
& 45.8\scriptsize$\pm1.8$ & 38.9\scriptsize$\pm0.8$ & 22.6\scriptsize$\pm1.0$
& 4.58\scriptsize$\pm0.5$ & 6.12\scriptsize$\pm0.5$ & \bf 1.09\scriptsize$\pm0.1$ \\
& ConceptNet 
& 13.4\scriptsize$\pm0.8$ & 15.5\scriptsize$\pm0.5$ & 4.74\scriptsize$\pm0.3$ 
& 54.0\scriptsize$\pm1.7$ & 43.3\scriptsize$\pm0.9$ & 26.9\scriptsize$\pm1.1$
& 1.31\scriptsize$\pm0.1$ & 2.25\scriptsize$\pm0.3$ & 0.34\scriptsize$\pm0.0$ \\
& \ours\ (ours)  
% & \bf 16.3\scriptsize$\pm0.3$ & \bf 17.8\scriptsize$\pm0.2$ & \bf 5.76\scriptsize$\pm0.1$
& \bf 16.6\scriptsize$\pm0.3$ & \bf 17.4\scriptsize$\pm0.6$ & \bf 5.76\scriptsize$\pm0.2$
& \bf 56.7\scriptsize$\pm1.3$ & \bf 43.9\scriptsize$\pm0.9$ & \bf 30.0\scriptsize$\pm1.1$
& \bf 4.63 & \bf 6.28 & \bf 1.09  \\
% & \bf 58.91 & \bf 44.54 & \bf 29.30 
% & 3.93 & 5.74 & 0.92 \\
% & - 
% & - & - & - & - 
% & - & - & - & - 
% & - & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{
% \update{
Quantitative results comparing Glove and ConceptNet with our FLM on MIT-States, UT-Zappos and C-GQA. We report unseen class accuracy (U), harmonic mean (H) and AUC using the CLIP, CoOp and CSP as CZSL base models.
% } 
\todo{add CGQA standard deviation.}
}
\vspace{-10pt}
\label{table:main_wo_seen}
\end{table*}

==> tables/rebuttal_all_seen.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{llccc|ccc|ccc}
\toprule
\bf{ViT-L/14} & & \multicolumn{3}{c|}{MIT-States} & \multicolumn{3}{c|}{UT-Zappos} & \multicolumn{3}{c}{C-GQA} \\ \hline
VLM & Method & U & H & AUC & U & H & AUC & U & H & AUC \\
\hline
\multirow{2}{*}{CLIP [20]}
& 200 seen pairs
& 11.70
& 11.03
& 2.45
& 21.42
& 10.25
& 1.68
& 2.27
& 2.85
& 0.15 \\
& LMFS (ours)
& \bf 13.79
& \bf 13.00
& \bf 3.08
& \bf 25.17
& \bf 11.49
& \bf 1.94
& \bf 2.53
& \bf 3.06
& \bf 0.16 \\
\hline
\multirow{2}{*}{CoOp [30]}
& 200 seen pairs
& 15.45
& 15.22
& 4.26
& 43.68
& 37.14
& 22.04
& 4.55
& 6.48
& 0.97 \\
& LMFS (ours)
& \bf 17.89
& \bf 16.99
& \bf 5.08
& \bf 51.82
& \bf 42.25
& \bf 26.68
& \bf 5.24
& \bf 7.02
& \bf 1.10 \\
\hline
\multirow{2}{*}{CSP [14]}
& 200 seen pairs
& 13.28
& 15.00
& 4.60
& 56.69
& 44.30
& 28.35
& 3.32
& 4.76
& 0.73 \\
& LMFS (ours)
& \bf 16.02
& \bf 17.43
& \bf 5.68
& \bf 58.91
& \bf 44.54
& \bf 29.30
& \bf 3.93
& \bf 5.74
& \bf 0.92 \\
\bottomrule
\end{tabular}
}
\caption{Using a maximum number of seen pairs in the guidance prompt.}
\vspace{-10pt}
\label{table:main}
\end{table*}

==> tables/rebuttal_calibrate.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{llccc|ccc|ccc}
\toprule
\bf{ViT-L/14} & & \multicolumn{3}{c|}{MIT-States} & \multicolumn{3}{c|}{UT-Zappos} & \multicolumn{3}{c}{C-GQA} \\ \hline
VLM & Method & U & H & AUC & U & H & AUC & U & H & AUC \\
\hline
\multirow{3}{*}{CLIP [20]} 
& ''no or yes``
& 13.66
& 12.39
& 2.88
& 21.21
& 11.07
& 1.73
& 2.19
& 2.61
& 0.13 \\
& Score 0 - 9
& 9.24
& 8.97
& 1.84
& 24.38
& 11.32
& 1.92
& 2.10
& 2.55
& 0.13 \\
& LMFS (ours, ``yes or no'')
& \bf 13.79
& \bf 13.00
& \bf 3.08
& \bf 25.17
& \bf 11.49
& \bf 1.94
& \bf 2.53
& \bf 3.06
& \bf 0.16 \\
\hline
\multirow{3}{*}{CoOp [30]}
& ``no or yes''
& 16.87
& 16.61
& 4.81
& 45.95
& 39.61
& 23.69
& 4.90
& 6.83
& 1.04 \\
& Score 0 - 9
& 13.09
& 13.66
& 3.63
& 46.27
& 43.75
& 26.17
& 4.72
& 6.37
& 0.95 \\
& LMFS (ours, ``yes or no'')
& \bf 17.89
& \bf 16.99
& \bf 5.08
& \bf 51.82
& \bf 42.25
& \bf 26.68
& \bf 5.24
& \bf 7.02
& \bf 1.10 \\
\hline
\multirow{3}{*}{CSP [14]}
& ``no or yes''
& 15.04
& 16.28
& 5.20
& 55.47
& 42.50
& 27.25
& 2.62
& 4.04
& 0.60 \\
& Score 0 - 9
& 11.31
& 13.01
& 3.79
& 53.83
& 44.99
& 29.01
& 2.27
& 3.56
& 0.51 \\
& LMFS (ours, ``yes or no'')
& \bf 16.02
& \bf 17.43
& \bf 5.68
& \bf 58.91
& \bf 44.54
& \bf 29.30
& \bf 3.93
& \bf 5.74
& \bf 0.92 \\
\bottomrule
\end{tabular}
}
\caption{LMFS using prompt variations to investigate logit calibration.}
\vspace{-10pt}
\label{table:main}
\end{table*}

==> tables/rebuttal_neg_examples.tex <==
\begin{table*}[t]
\centering
% \setlength{\tabcolsep}{3pt}
% \resizebox{\textwidth}{!}
% {
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{llccc}
\toprule
\bf{ViT-L/14} & & \multicolumn{3}{c}{MIT-States} \\ \hline
VLM & Method & S & U & H \\
\hline
\multirow{5}{*}{CSP [14]}
& pos only (L326-339) & 14.04 & 15.59 & 4.95 \\
& pos-neg order & 13.21 & 14.75 & 4.51 \\
& neg-pos order & 12.17 & 13.89 & 4.11 \\
& pos/neg random order & 12.73 & 14.26 & 4.33 \\
& LMFS (ours) & \bf 16.02 & \bf 17.43 & \bf 5.68 \\
\bottomrule
\end{tabular}
% }
\caption{Using both positive and negative examples in the guidance prompt.}
\vspace{-10pt}
\label{table:main}
\end{table*}

==> tables/rebuttal_obj_state_acc.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{llcccc|cccc|cccc}
\toprule
\bf{ViT-L/14} & & \multicolumn{4}{c|}{MIT-States} & \multicolumn{4}{c|}{UT-Zappos} & \multicolumn{4}{c}{C-GQA} \\ \hline
VLM & Method 
& \begin{tabular}[c]{@{}c@{}}Attr.\\acc.\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}Obj.\\acc.\end{tabular}  
& H   
& AUC 
& \begin{tabular}[c]{@{}c@{}}Attr.\\acc.\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}Obj.\\acc.\end{tabular}    
& H 
& AUC 
& \begin{tabular}[c]{@{}c@{}}Attr.\\acc.\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}Obj.\\acc.\end{tabular}  
& H 
& AUC \\
\hline
\multirow{3}{*}{CLIP [20]} 
& CompCos [9]
& \bf 22.45
& 47.17
& \bf 13.01 
& 3.08
& 20.97
& 52.78
& 10.6
& 1.59
& \bf 12.46
& \bf 29.84
& 2.46
& \bf 0.20 \\
& KGSP [6]
& 21.88
& 45.96
& 12.65
& 2.75
& 19.94
& \bf 54.32
& 10.32
& 1.69
& 7.40
& 26.42
& 2.59
& 0.13 \\
& LMFS (ours)
& 22.09
& \bf 47.65
& 13.00
& \bf 3.08
& \bf 22.03
& 53.33
& \bf 11.49
& \bf 1.94
& 10.18
& 28.64
& \bf 3.06
& 0.16 \\
\hline
\multirow{3}{*}{CoOp [30]}
& CompCos [9]
& 24.82
& 50.23
& 15.91
& 4.67
& 47.29
& 72.37
& 36.22
& 19.81
& 22.11
& \bf 40.62
& 6.25
& 0.98 \\
& KGSP [6]
& 24.29
& 49.67
& 15.76
& 4.35
& 47.08
& 71.45
& 37.00
& 21.91
& 19.22
& 38.54
& 6.16
& 0.93 \\
& LMFS (ours)
& \bf 25.33
& \bf 51.18
& \bf 16.99
& \bf 5.08
& \bf 53.09
& \bf 73.99
& \bf 42.25
& \bf 26.68
& \bf 22.13
& 40.29
& \bf 7.02
& \bf 1.10 \\
\hline
\multirow{3}{*}{CSP [14]}
& CompCos [9]
& 26.28
& 49.80
& 16.82
& 5.30
& 49.86
& 75.36
& 39.47
& 24.01
& \bf 23.32
& \bf 42.90
& \bf 5.81
& \bf 1.03 \\
& KGSP [6]
& 25.44
& 49.22
& 16.34
& 5.22
& 53.36
& 76.66
& 44.33
& 28.39
& 18.22
& 38.88
& 2.12
& 0.32 \\
& LMFS (ours)
& \bf 26.67
& \bf 50.32
& \bf 17.43
& \bf 5.68
& \bf 54.12
& \bf 77.25
& \bf 44.54
& \bf 29.30
& 16.87
& 39.96
& 5.74
& 0.92 \\
\bottomrule
\end{tabular}
}
\caption{Attribute and object accuracies.}
\vspace{-10pt}
\label{table:main}
\end{table*}
